A Parametric Study of the SASI Comparing General Relativistic and Nonrelativistic Treatments

We present numerical results from a parameter study of the standing accretion shock instability (SASI), investigating the impact of general relativity (GR) on the dynamics. Using GR hydrodynamics with GR gravity, and nonrelativistic (NR) hydrodynamics with Newtonian gravity, in an idealized model setting, we vary the initial radius of the shock and, by varying its mass and radius in concert, the proto-neutron star (PNS) compactness. We investigate four compactnesses expected in a post-bounce core-collapse supernova (CCSN). We find that GR leads to a longer SASI oscillation period, with ratios between the GR and NR cases as large as 1.29 for the highest-compactness suite. We also find that GR leads to a slower SASI growth rate, with ratios between the GR and NR cases as low as 0.47 for the highest-compactness suite. We discuss implications of our results for CCSN simulations.

==> resultsTable.tex <==
\begin{deluxetable}{cccccc}[ht]
  \tablecaption{Results}
  \tablehead %
  { %
  \colhead{Model}                                          &
  \colhead{$T\pm\Delta T\,\left[\ms\right]$}               &
  \colhead{$\omega\pm\Delta\omega\,\left[\ms^{-1}\right]$} &
  \colhead{$\omega\,T$}                                    &
  \colhead{$\taa\,\left[\ms\right]$}                       &
  \colhead{$\tac\,\left[\ms\right]$}                       %
  }
  \startdata
  \texttt{NR\_M1.4\_Rpns070\_Rs1.50e2} & 25.5566 $\pm$ 21.1850 & 0.0631 $\pm$ 0.0011 & 1.6123 & 20.9559 & 36.6791 \\
  \texttt{GR\_M1.4\_Rpns070\_Rs1.50e2} & 30.3854 $\pm$ 21.5598 & 0.0603 $\pm$ 0.0009 & 1.8313 & 22.6462 & 37.4293 \\
  \texttt{NR\_M1.4\_Rpns040\_Rs1.20e2} & 24.6398 $\pm$ 15.6904 & 0.0733 $\pm$ 0.0011 & 1.8054 & 20.8348 & 26.2646 \\
  \texttt{GR\_M1.4\_Rpns040\_Rs1.20e2} & 27.2758 $\pm$ 16.6796 & 0.0578 $\pm$ 0.0011 & 1.5758 & 23.6236 & 26.9372 \\
  \texttt{NR\_M1.4\_Rpns040\_Rs1.50e2} & 37.3656 $\pm$ 23.4864 & 0.0409 $\pm$ 0.0005 & 1.5291 & 34.3279 & 36.6791 \\
  \texttt{GR\_M1.4\_Rpns040\_Rs1.50e2} & 42.9166 $\pm$ 22.4149 & 0.0360 $\pm$ 0.0004 & 1.5461 & 38.6747 & 37.4293 \\
  \texttt{NR\_M1.4\_Rpns040\_Rs1.75e2} & 51.5463 $\pm$ 29.2280 & 0.0300 $\pm$ 0.0003 & 1.5468 & 47.7212 & 46.0841 \\
  \texttt{GR\_M1.4\_Rpns040\_Rs1.75e2} & 58.6525 $\pm$ 28.1381 & 0.0265 $\pm$ 0.0003 & 1.5540 & 53.5372 & 46.8924 \\
  \texttt{NR\_M1.8\_Rpns020\_Rs7.00e1} & 9.8537 $\pm$ 5.1860 & 0.1524 $\pm$ 0.0039 & 1.5016 & 9.2361 & 10.3138 \\
  \texttt{GR\_M1.8\_Rpns020\_Rs7.00e1} & 12.0565 $\pm$ 4.6944 & 0.1031 $\pm$ 0.0022 & 1.2429 & 12.6159 & 10.9053 \\
  \texttt{NR\_M2.8\_Rpns020\_Rs6.00e1} & 6.1939 $\pm$ 3.7227 & 0.2910 $\pm$ 0.0085 & 1.8027 & 5.2343 & 6.5656 \\
  \texttt{GR\_M2.8\_Rpns020\_Rs6.00e1} & 7.5296 $\pm$ 2.5224 & 0.1365 $\pm$ 0.0042 & 1.0282 & 8.6607 & 7.2635 \\
  \texttt{NR\_M2.8\_Rpns020\_Rs7.00e1} & 7.9137 $\pm$ 4.2711 & 0.1897 $\pm$ 0.0054 & 1.5014 & 7.4177 & 8.2693 \\
  \texttt{GR\_M2.8\_Rpns020\_Rs7.00e1} & 10.2013 $\pm$ 3.0563 & 0.0954 $\pm$ 0.0026 & 0.9735 & 12.1099 & 9.0178 \\
  \enddata
  \label{tab.results}
  \tablecomments{
Oscillation periods, growth rates, and their uncertainties for all
fourteen models having the same accretion rate of $0.3\,\msun\,\s^{-1}$.
\repl{The first six are the low-compactness models; the last four
are the high-compactness models.}{}
The uncertainties for the growth rates are defined as the square roots of the
diagonal entries of the covariance matrix corresponding to the growth rate.
The uncertainies for the oscillation period are defined as the full-width
half-maximum values of the Fourier amplitudes (see \figref{fig.fft}).
The fourth column shows the product of the best-fit growth rate multiplied
by the best-fit oscillation period.
The fifth column shows the estimate for the period assuming an
advective-acoustic origin of the SASI \myeqref{eq.MullerEst},
and the sixth column shows the estimate for the period assuming
a purely acoustic origin of the SASI \myeqref{eq.Tac}, where we use
$\rac=0.85\,\rsh$, the midpoint
of the shell in which we compute the power (see \secref{sec.results}).}
\end{deluxetable}
